Modelling Cellular Perturbations with the Sparse Additive Mechanism Shift Variational Autoencoder

Generative models of observations under interventions have been a vibrant topic of interest across machine learning and the sciences in recent years. For example, in drug discovery, there is a need to model the effects of diverse interventions on cells in order to characterize unknown biological mechanisms of action. We propose the Sparse Additive Mechanism Shift Variational Autoencoder, SAMS-VAE, to combine compositionality, disentanglement, and interpretability for perturbation models. SAMS-VAE models the latent state of a perturbed sample as the sum of a local latent variable capturing sample-specific variation and sparse global variables of latent intervention effects. Crucially, SAMS-VAE sparsifies these global latent variables for individual perturbations to identify disentangled, perturbation-specific latent subspaces that are flexibly composable. We evaluate SAMS-VAE both quantitatively and qualitatively on a range of tasks using two popular single cell sequencing datasets. In order to measure perturbation-specific model-properties, we also introduce a framework for evaluation of perturbation models based on average treatment effects with links to posterior predictive checks. SAMS-VAE outperforms comparable models in terms of generalization across in-distribution and out-of-distribution tasks, including a combinatorial reasoning task under resource paucity, and yields interpretable latent structures which correlate strongly to known biological mechanisms. Our results suggest SAMS-VAE is an interesting addition to the modeling toolkit for machine learning-driven scientific discovery.

==> tables/table1.tex <==
\begin{table}[t!]
    \centering
    % \setlength{\tabcolsep}{8pt}
    \small
    \caption{Test accuracy of 160-way perturbed gene prediction on JUMP-CP. Two training settings are considered: one using only 5 fluorescence channels and the other incorporating all 8 channels, which includes 3 additional brightfield channels. During testing, all possible channel combinations are evaluated and we report the mean accuracies for combinations with the same number of channels (See Appendix~\ref{app:extra} for detailed error analyses). We observe that cross channel reasoning is crucial when the inputs have independent information (fluorescence vs. brightfield). 
    }
    \vspace{-2mm}
    \label{tab:jumpcp}
    \begin{tabular}{llcccccc}
        \toprule
        % \midrule
        Model & Test IWELBO & Mask PW. Acc. & ATE Pearson \\
        & Model & Test IWELBO & Mask PW. Acc. & ATE Pearson \hspace{-2mm} \\
        \cmidrule(lr){3-8}
        \multicolumn{2}{c}{\begin{tabular}{@{}c@{}}Use hierarchical\\channel sampling?\end{tabular}}\hspace{-2mm}
        & \xmark & \xmark & \cmark & \cmark & \cmark & \cmark \\        \midrule
\multicolumn{7}{l}{\emph{Training on 5 fluorescence channels}}\vspace{1mm} \\
\multirow{5}{*}{\rotatebox[origin=c]{90}{\begin{tabular}{@{}c@{}}\#channels\vspace{-1mm} \\for testing\end{tabular}}} \hspace{-4mm}
& 5 channels                & 48.41 & 53.41 & 55.51 & 56.78 & \textbf{60.29} & 60.03 \\
& 4 channels                & 0.85  & 15.13 & 43.59 & 45.94 & 48.80 & \textbf{49.34} \\
& 3 channels                & 1.89  &  5.12 & 33.14 & 35.45 & 37.13 & \textbf{38.15} \\
& 2 channels                & 1.46  &  1.22 & 25.24 & 26.57 & 27.40 & \textbf{27.99} \\
& 1 channel{\phantom{s}}    & 0.54  &  1.25 & 20.49 & 21.43 & 21.30 & \textbf{21.58} \\\midrule
\multicolumn{7}{l}{\emph{Training on all 8 channels (5 fluorescence channels \& 3 brightfield channels)}}\vspace{1mm} \\
\multirow{8}{*}{\rotatebox[origin=c]{90}{\begin{tabular}{@{}c@{}}\#channels\vspace{-1mm} \\for testing\end{tabular}}} \hspace{-4mm}
& 8 channels                & 52.06 & 66.22 & 56.87 & 68.09 & 66.44 & \textbf{74.77} \\
& 7 channels                &  5.91 & 41.03 & 49.35 & 61.02 & 59.01 & \textbf{68.42} \\
& 6 channels                &  1.81 & 24.57 & 42.38 & 53.45 & 51.29 & \textbf{61.26} \\
& 5 channels                &  2.46 & 14.20 & 35.78 & 45.50 & 43.39 & \textbf{53.05} \\
& 4 channels                &  2.38 &  8.56 & 29.84 & 37.37 & 35.60 & \textbf{43.87} \\
& 3 channels                &  2.70 &  5.65 & 24.94 & 29.68 & 28.59 & \textbf{34.19} \\
& 2 channels                &  2.63 &  3.24 & 21.54 & 23.77 & 23.32 & \textbf{25.73} \\
& 1 channel{\phantom{s}}    &  3.00 &  2.08 & 19.92 & 20.84 & 20.41 & \textbf{21.20} \\
        % \midrule
        \bottomrule
    \end{tabular}
    \vspace{-4mm}
\end{table}






==> tables/table_replogle.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        Model & Test IWELBO & Mask Pathway Prediction Acc. \\
        \hline
        Conditional VAE & $-1765.91 \pm 0.24$ & - \\
        \hline
        SVAE+ & $-1759.61 \pm 0.23 $ & $0.69 \pm 0.05$ \\
        \hline
        CPA-VAE (mean field) & $-1760.06 \pm 0.24$ & - \\
        CPA-VAE (correlated $z_{basal}$) & $-1756.72 \pm 0.38$ & - \\
        \hline
        SAMS-VAE (mean field) & $-1757.70 \pm 0.11$ & $ 0.78 \pm 0.03 $ \\
        SAMS-VAE (correlated $E$) & $-1757.93 \pm 0.09$ & \boldmath$0.90 \pm 0.04$ \\
        SAMS-VAE (correlated $z_{basal}$) & $-1756.23 \pm 0.05$ & $0.83 \pm 0.02$ \\
        SAMS-VAE (correlated $z_{basal}$ and $E$) & \boldmath$-1756.11 \pm 0.08$ & \boldmath$0.90 \pm 0.02$ \\
        \hline
    \end{tabular}
    \caption{Quantitative evaluation of models on Replogle filtered dataset (100 latent dimensions)}
    \label{table:replogle-quantitative}
\end{table}

==> tables/table_replogle_ATE.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        Model & Test IWELBO & Mask PW. Acc. & ATE Pearson \\
        \hline
        Conditional VAE & $-1765.91 \pm 0.24$ & - & \boldmath$0.758636	\pm 0.006$ \\
        \hline
        SVAE+ & $-1759.61 \pm 0.23 $ & $0.69 \pm 0.05$ & $0.600834	\pm 0.013$ \\
        \hline
        CPA-VAE (mean field) & $-1760.06 \pm 0.24$ & - & $0.4893	\pm 0.018$ \\
        CPA-VAE (corr. $z_{basal}$) & $-1756.72 \pm 0.38$ & - & $0.559705	\pm 0.016$ \\
        \hline
        SAMS-VAE (mean field) & $-1757.70 \pm 0.11$ & $ 0.78 \pm 0.03 $ & $0.26914 \pm 0.004$\\
        SAMS-VAE (corr. $E$) & $-1757.93 \pm 0.09$ & \boldmath$0.90 \pm 0.04$ & $0.312267 \pm 0.002$ \\
        SAMS-VAE (corr. $z_{basal}$) & $-1756.23 \pm 0.05$ & $0.83 \pm 0.02$ & $0.736357	\pm 0.013$\\
        SAMS-VAE (corr. $z_{basal}$ and $E$) & \boldmath$-1756.11 \pm 0.08$ & \boldmath$0.90 \pm 0.02$ & \boldmath$0.74373 \pm 0.018$\\
        \hline
    \end{tabular}
    \caption{Quantitative evaluation of models on Replogle filtered dataset (100 latent dimensions)}
    \label{table:replogle-ATE-old}
\end{table}

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}
